Synchronization and Phase Noise Reduction in Micromechanical Oscillators Arrays Coupled through Light

Synchronization of many coupled oscillators is widely found in nature and has the potential to revolutionize timing technologies. Here we demonstrate synchronization in arrays of silicon nitride micromechanical oscillators coupled purely through optical radiation field. We show that the phase noise of the synchronized oscillators can be improved by almost 10 dB below the phase noise limit for each individual oscillator. These results open a practical route towards synchronized oscillator networks.

==> multisync_supp_arxiv.tex <==

%Setup counters for supplementary
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{equation}{0}

\subsection{Optical Transmission}

\begin{figure}[!h]
  \centering
  \includegraphics[angle=0,width=0.6\textwidth]{cwandccw_final.pdf}
\caption{Mode excitation geometry (a) In a square lattice, only one direction of the optical mode is excited. (b) In a triangular lattice, the coupling geometry determines that as the light from the waveguide excites the clockwise mode of OMO 1 which in turn excites the counter-clockwise mode of OMO 2 and OMO 3. However, the counter-clockwise mode of OMO 3 also excite the clockwise mode of OMO 2 (blue arrow), which therefore excites all the counter propagating wave of the entire system.}
\label{fig:cwccw}
\end{figure}

The challenge in optically coupling large arrays of mechanical structures is the variation of the optical frequencies of each individual OMO due to variation in the exact fabricated dimensions. This can be in principle compensated by integrating optical tuning mechanisms such as heaters. In our device, we overcome this challenge by ensuring that the optical coupling is large compare to the frequency variation and the individual decay rate of each cavity. The optical coupling strength we designed ($\kappa_{(i,j)}\sim 5$ GHz) is much larger than the optical decay rate of the cavity ($\gamma_i \sim 400$ MHz) and to the cavity optical frequency spread from fabrication variations ($\Delta\omega<2$ GHz). This ensures that the optical modes are strongly coupled which means the light travels between the cavities many times before it is lost via other channels.

We estimate the spatial structure of the optical supermodes using coupled mode theory \cite{Hau84}. In the $2\times 2$ OMO array, the coupled modes can be solved essentially using the same method as described in previous work of two coupled double disk OMOs \cite{zhang_synchronization_2012}. The evolution and coupling of each individual optical mode is described by a matrix where its diagonal entries describe the eigenfrequencies and the off-diagonal entries describe the coupling between these modes. In the case for the three- and seven- OMO arrays arranged in a triangular lattice, we must consider both the clock-wise and counter-clock wise optical modes, as both will be excited through a laser coupled to one direction even without any backscatters (Fig. \ref{fig:cwccw}). 

\begin{figure}
  \centering
  \includegraphics[angle=0,width=1\textwidth]{optical_trans_final.pdf}

\caption{The optical transmission in the (a) three,  (b)four and (c) seven cavity arrays respectively. The well split resonant mode and the high extinction of each split supermodes shows that the optical modes are strongly coupled.}
  \label{fig:opttrans}
\end{figure}
The coupled mode equation that governs the optical part reads
 
\begin{equation}
\begin{aligned}
\label{eq:opt_diagonal}
\left(\begin{array}{c}
\dot{a}_{1}\\
\dot{a}_{2}\\
...\\
\dot{a}_{i}\\
...\\
\dot{a}_{n}
\end{array}\right)&=
\left(
\begin{array}{cccccc}
 -\frac{\gamma _1}{2}-\mathrm{i} \omega _1 & \frac{\mathrm{i} \kappa_{12} }{2} & ... & \frac{\mathrm{i} \kappa_{1i} }{2} & ... & \frac{\mathrm{i} \kappa_{1n} }{2} \\
 \frac{\mathrm{i} \kappa_{21}}{2} & -\frac{\gamma _2}{2}-\mathrm{i} \omega _2 & ... & \frac{\mathrm{i} \kappa_{2i}}{2} & ... & \frac{\mathrm{i} \kappa_{2n} }{2} \\
 ... & ... & ... & ...& ... & ...\\
 \frac{\mathrm{i} \kappa_{i1} }{2} & \frac{\mathrm{i} \kappa_{i2} }{2} & ... & -\frac{\gamma _i}{2}-\mathrm{i} \omega _i& ... &  \frac{\mathrm{i} \kappa_{in} }{2}\\
 ... & ... & ... & ...& ... & ...\\
 \frac{\mathrm{i} \kappa_{n1} }{2} & \frac{\mathrm{i} \kappa_{n2} }{2} & ... & \frac{\mathrm{i} \kappa_{in} }{2}& ... & -\frac{\gamma _n}{2}-\mathrm{i} \omega _n\\
\end{array}\right)
\left(\begin{array}{c}
{a}_{1}\\
{a}_{2}\\
...\\
{a}_{i}\\
...\\
\dot{a}_{n}
\end{array}\right)
+\sqrt{\gamma _1 \eta _{c}}s(t) 
\left(\begin{array}{c}
1\\
0\\
...\\
0\\
...\\
0
\end{array}\right)
\end{aligned}
\end{equation}

where $\gamma_i, \omega_i$ are the total damping rate and the resonant frequency of each individual optical mode $a_i$. $\kappa_{ij}$ is the optical coupling strength between $i$th and $j$th OMO. $|s(t)|^2$ is the optical power that excites the array of resonators through the first cavity. $\eta_c$ is the optical criticality factor, the ratio between the cavity damping rate and the external coupling rate. For triangular lattice cases, the matrix dimension is increased from $n$ to $2n$ where the both the cw and ccw degrees of freedoms are taken into account. In the strong coupling regime ($\kappa_{ij}\gg\gamma_i ~\forall i,j$), individual optical modes hybridize and fully splits into optical supermodes $b_m$ where some supermodes span over all cavities. The spatial geometry of these supermodes can be analyzed through rewriting equation \ref{eq:opt_diagonal} in the optical supermode basis $b_m = \sum\limits_{i=1}^{N}c_i a_i$ where $c_i$ indicates the relative optical field amplitude in cavity $i$. To conveniently visualize the spatial geometry of the optical supermode, we approximate $\gamma_i$ and $\Omega_i$ of individual OMO being identical. We can then exactly diagonalize the coupling matrix in equation \ref{eq:opt_diagonal} through Jordan matrix decomposition to find the new optical supermodes basis $b_m$ in superposition of the individual optical mode $a_i$. The geometric representation of the superposition is shown in figure 2 in the main text. 

Figure \ref{fig:mult_IR} shows images from the IR camera when the supermodes spanning over all cavities are excited. It is clear from the image that all cavities light up with approximately equal intensities. The strong coupling is also visualized by the fully split optical supermodes shown in the optical transmission in figure \ref{fig:opttrans}.

\begin{figure}
  \centering

  \includegraphics[angle=0,width=0.8\textwidth]{IR_image_final.pdf}
\caption{Image of the scattered light when sychronization is onset for (a) three-cavity (b) four-cavity and (c) seven-cavity arrays. The scale bars are 20 $\mu$m.}
  \label{fig:mult_IR}
\end{figure}

\subsection{Mechanical modes}
The mechanical modes of the double disk are the flapping mechanical mode where we can control the mechanical frequency of the mode by the undercut depth of the sacrificial silicon dioxide layer. In the particular device we used in the experiment, we fabricated the devices with mechanical frequencies near 132.5 MHz and quality factor near 1000 (Fig. \ref{fig:mult_mech}). Typical optical quality factor of these devices is $\sim$ 500,000. interaction strength between the optical and the mechanical mode is characterized by the optomechanical coupling strength $g_{\rm{om}}=\frac{d\omega}{dx}=2\pi\times 50 $ GHz/nm for our devices \cite{zhang_synchronization_2012}.

In the OMO arrays, when the system is coupled to a laser at very low power, we measure a distribution of mechanical frequencies corresponding to different OMOs. Figure \ref{fig:mult_mech2} shows the mechanical spectrum in the three, four and seven cavity arrays respectively. In the three OMO array, the mechanical frequencies are clearly different whereas in the four and seven OMO arrays, the mechanical mode frequencies are different but also overlapping.

\begin{figure}
  \centering

  \includegraphics[angle=0,width=0.8\textwidth]{mech_spec_single_final2.pdf}
\caption{(a) Thermal mechanical spectrum of a single doubled-disk OMO forming the array in this experiment. (b) Self-sustaining oscillation spectrum of a single double-disk OMO.}
  \label{fig:mult_mech}
\end{figure}

\begin{figure}[!h]
  \centering

  \includegraphics[angle=0,width=1\textwidth]{mech_spec_final.pdf}
\caption{The mechanical spectrum in the (a) three,  (b)four and (c) seven cavity arrays at low optical powers respectively. The disorder in mechanical frequencies is evident from the splitting of the peaks.}
  \label{fig:mult_mech2}
\end{figure}
 %---------------------------------------------------------------
 %Experimental Setup
 %---------------------------------------------------------------
\subsection{Phase Noise}
We measure the phase noise of our oscillator by feeding the output of the photodiode (New Focus 1811) to a spectrum analyzer (Agilent E4407B). To measure the phase noise at 10 kHz offset frequency, we utilize the spot frequency measurement option in the phase noise measurement module (Option 226) of the spectrum analyzer which enables fast noise spectral power measurement at a single offset frequency. 

In synchronized oscillator arrays, the phase noise reduces as the number of synchronized oscillators increase. Experiments and theories \cite{chang_phase_1997,pikovsky_synchronization:_2003} show that the noise reduces as $1/N$ where $N$ is the number of synchronized oscillators. This can be intuitively understood as coordinated oscillators while having the same frequency but having an increased effective mass which improves their resistance to thermomechanical fluctuations. In our system, proving synchronization by studying the dynamics of individual cavities in the arrays is desirable but it is technically challenging given the compact size of the array. Therefore we choose the phase noise as a figure of merit as it is fundamentally limited by the thermomechanical process. 

The phase noise performance of an optomechanical oscillator, when limited by thermomechanical noise, improves when the laser power is increased. At high laser driving powers, the phase noise roughly stays constant as the laser power is further increased.  We calibrate the single oscillator phase noise performance by measuring the phase noise at 10 kHz carrier offset at different laser driving powers. Figure \ref{fig:pn_one} clear shows that the phase noise does not vary significantly when the power is above $4\times P_{th}$. where $P_{\rm{th}}=10 ~\mu$W is the typical threshold power for a single OMO. This is in agreement with the experimental observation reported by Mani et. al \cite {hossein-zadeh_characterization_2006}. and theory by Fong et. al \cite{fong_phase_2014}.

%We experimentally characterize a single double-disk optomechanical oscillator. We obtain the mechanical quality factor through a fitting the RF spectrum of the optical transmission in a low power measurement. The fitted mechanical quality factor is $Q_m=(1190\pm 20)$. When the OMO is driven into self-sustained oscillation, it produces a sharp peak at the oscillation frequency of the mechanical oscillator. We detect this signal on a square-law photodetector which replicates the mechanical motion of the cantilevers. Figure SX shows the dependence of phase noise at large carrier offset verses optical driving power. It is clear from the measurements that the phase noise improves very slowly at large optical driving powers. In all our phase noise measurements, we choose the optical powers such that they well exceed the threshold power of self-oscillations and yet are still close to each other ($P_{in}\sim 30-50 P_{th}$). %

\begin{figure}
  \centering
  \includegraphics[angle=0,width=0.5\textwidth]{phase_noise_oneosc_final.pdf}
\caption{Spot frequency phase noise of a single OMO at 10 kHz offset from the carrier frequency as a function of laser power. $P_{\rm{th}}=10 ~\mu$W is the threshold power for a single OMO to oscillate.}
  \label{fig:pn_one}
\end{figure}


\begin{figure}
  \centering
  \includegraphics[angle=0,width=0.8\textwidth]{mech_sim_final.pdf}
\caption{FEM simulation of the mechanical mode. (a) Geometry of the structure. (b) Simulated mechanical displacement profile. The antisymmetric mechanical mode simulated has a vibration frequency of 131 MHz with an effective mass of 70 pg.}
  \label{fig:mech_sim}
\end{figure}

%We will see that for an OMO where the mechanical oscillation is limited by the nonlinearity in the optomechanical transfer function, the linewidth of the oscillation signal does not vary significantly as the optical power gets very large. This can be simply understood as the following. The mechanical oscillator acquires energy from the optical field losses energy through mechanical damping to the environment and establish a stable limit cycle. The maximum amount of energy the OMO could possibly acquire should be limited by the total power dropped in optical cavity throughout the mechanical oscillation cycle. As the mechanical oscillator vibrates, the optical frequency shifts according to
%\begin{equation}
%\omega=\omega_0+g_\textnormal{om} x
%\end{equation}
%where $\omega_0$ is the natural frequency of the optical resonance and $g_\textnormal{om}$ is a constant linearly relates the mechanical displacement to the frequency of the %cavity ($\omega$). For large value of $x$, the total optical power coupled into the optical resonator ($P_textnormal{tot}$)in half a period of a mechanical oscillation is
%\begin{equation}
%P_\textnormal{tot}(x_0) = \int\limits_{-x_0}^{x_0}\frac{|s_\textnormal{in}|^2 \kappa_\textnormal{ext}}{(\omega_0+g_\textnormal{om} x-\omega_L)^2+\kappa_o^4}
%\end{equation}
%where $x_0$ is the amplitude of the mechanical oscillation, $s_\textnormal{in}$ is the input optical field, $\kappa_\textnormal{ext}$ is the cavity field coupling rate, $\omega_L$ is the laser wavelength and $\kappa_o$ is the optical cavity damping rate. We could easily observe the dependence of the mechanical amplitude to optical power $x_0(P_\textnormal{tot})$ by graphically plot the inverse of the above integral function. %
Leeson’s model \cite{leeson_simple_1966} predicts the phase noise of self-sustaining oscillators from the linewidth of the oscillation signal. The linewidth ($\Delta \Omega$) of a thermally limited oscillator is given by
\begin{equation}
\label{eq:linwid}
\Delta \Omega = \frac{k_B T}{2 P_\textnormal{out}}\Gamma_m^2
\end{equation}
where $k_B$ is Boltzmann's constant, $T$ is the temperature, $P_\textnormal{out}$ is the output power of the oscillator and $\Gamma_m$ is the natural damping rate of the oscillator. Since the double disk we use have a small effective mass $m_\textnormal{eff}$ (Fig. \ref{fig:mech_sim}), which means a low oscillator power, the phase noise is limited by thermomechanical noise. The oscillator power $P_\textnormal{out}$ is given by,

\begin{equation}
P_\textnormal{out} = \frac{1}{2}m_\textnormal{eff}\Omega^2 x^2 \Gamma_m
\end{equation}

where $x$ is the maximum displacement amplitude of the oscillator. Equation \eqref{eq:linwid} can be represented as,
\begin{equation}
\label{eq:linwidexp}
\Delta \Omega = \frac{k_B T}{ m_\textnormal{eff}\Omega^2 x^2}\Gamma_m
\end{equation}

In our experiment, since the offset frequency $\Delta f$ we are interested in is much larger than the linewidth ($\Delta \Omega$) of our oscillator, the phase noise $L(\Delta f)$ in dBc/Hz predicted by Leeson's equation\cite{leeson_simple_1966} can be simplified as,

\begin{equation}
\label{eq:lee}
L(\Delta f)=10 \textnormal{Log}_{10}\left(\frac{\Delta \Omega}{2\pi \Delta f^2}\right)
\end{equation}

Substituting the parameters ($T=300$ K; $m_\textnormal{eff}=70$ pg; $\Gamma_m=2\pi \times 110$ kHz) and $x\sim g_{om}/\gamma = 10$ pm to equation \ref{eq:lee}, we obtain a theoretical estimate of the thermomechanical noise limit of our oscillators which is $-60$ dBc/Hz at $10$ kHz carrier frequency offset in good agreement with our experimental measurements and previous frequency dependent phase noise measurements \cite{shah_master-slave_2015}. 

We expect the laser noise to be a minor contribution to the phase noise of our OMOs at 10 kHz carrier offset. Although diode lasers typically have relatively high phase noise, at this frequency, the phase noise of the laser is not relevant because the optical force is only affected by laser intensity. The cavity decay rate ($\frac{\gamma}{2\pi}\sim 400$ MHz) is much higher than 10 kHz which means the laser phase noise does not get converted in to intensity noise due to the cavity response. Typical relative intensity noise (RIN) of external cavity tunable laser at low frequencies is below -100 dBc/Hz \cite{laurila_tunable_2002}. We measure the RIN of the laser we use (Tunics Reference) at 50 $\mu$W to be -112 dBc/Hz at 10 kHz offset through the photodiode (New Focus 1811) and the spectrum analyzer (Agilent E4407B). As laser shot noise is much lower than technical noise at this laser power and frequency, we expect minimal contribution from the shot noise of the laser. Our analysis is consistent with previous theory \cite{fong_phase_2014}. \\

%\bibliographystyle{naturemag}
%\bibliography{synchronization}
